All Prime Numbers Have Primitive Roots

If p is a prime, then the numbers 1, 2, ..., p-1 form a group under multiplication modulo p. A number g that generates this group is called a primitive root of p; i.e., g is such that every number between 1 and p-1 can be written as a power of g modulo p. Building on prior work in the ACL2 community, this paper describes a constructive proof that every prime number has a primitive root.

==> eptcsdata.tex <==
\providecommand{\firstpage}{9}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.3}{10.4204/EPTCS.359.3}}
\pdfoutput=1

